Token-passing Optimal Reduction with Embedded Read-back

We introduce a new interaction net implementation of optimal reduction for the pure untyped lambda calculus. Unlike others, our implementation allows to reach normal form regardless of the interaction net reduction strategy using the approach of so-called token-passing nets and a non-deterministic extension for interaction nets. Another new feature is the read-back mechanism implemented without leaving the formalism of interaction nets.

==> eptcsdata.tex <==
\providecommand{\firstpage}{45}
\providecommand{\publicationstatus}{A. Corradini \& H. Zantema (Eds.)\\
Computing with Terms and Graphs (TERMGRAPH 2016)\\
EPTCS 225, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.225.7}{10.4204/EPTCS.225.7}}
\pdfoutput=1

